Large-scale Spatiotemporal Characterization of Inconsistencies in the World's Largest Firewall

A nation-scale firewall, colloquially referred to as the "Great Firewall of China," implements many different types of censorship and content filtering to control China's Internet traffic. Past work has shown that the firewall occasionally fails. In other words, sometimes clients in China are able to reach blacklisted servers outside of China. This phenomenon has not yet been characterized because it is infeasible to find a large and geographically diverse set of clients in China from which to test connectivity. In this paper, we overcome this challenge by using hybrid idle scan techniques that are able to measure connectivity between a remote client and an arbitrary server, neither of which are under the control of the researcher performing measurements. In addition to hybrid idle scans, we present and employ a novel side channel in the Linux kernel's SYN backlog. We demonstrate both techniques by measuring the reachability of the Tor network which is known to be blocked in China. Our measurements reveal that 1) failures in the firewall occur throughout the entire country without any conspicuous geographical patterns, 2) a network block in China appears to have unfiltered access to parts of the Tor network, and 3) the filtering seems to be mostly centralized at the level of Internet exchange points. Our work also answers many other open questions about the Great Firewall's architecture and implementation.

==> implementation.tex <==

%In this section, we describe our probing infrastructure, the challenges our
%measurement methodology was designed to address, and the measurement
%methodology for the measurements presented in Section~\ref{sec:results}.

All measurement machines were Linux machines connected to a research network
with no packet filtering.  Specifically, this network has no stateful firewall
or egress filtering for return IP addresses.
%Measurement machine IPs were not
%bound to any interfaces to eliminate unwanted packets being sent.

%A major challenge that we considered in our experimental methodology is that
%hosts sometimes do not stay up and alive throughout the whole experiment.
%Furthermore, because of DHCP and other factors, IP addresses can be bound to
%different hosts or not consistently exhibit behaviors that our method assumes
%(such as global IPIDs) throughout a full experiment.  Another challenge is that
%packet delay, packet loss, and the routes that packets take can vary throughout
%the day.  Thus it is important to avoid letting diurnal patterns affect the
%results.

One measurement machine was dedicated to developing a pool of both client and
server IP addresses that have the right properties for use in measurements.
Clients were chosen by horizontally scanning China and other countries for
machines with global IPIDs, then continually checking them for a 24-hour period
to cull out IP addresses that frequently changed global IPID behavior
(\emph{e.g.}, because of DHCP), went down, or were too noisy.  A machine is
considered to have a global IPID if its IPID as we measure it by sending
SYN/ACKs from alternating source IP addresses and receiving RSTs never
incrementing outside the ranges $[-40, 0)$ or $(0, 1000]$ per second when probed
from two different IP addresses.  This range allows for non-idle clients,
packet loss, and packet reordering.  It is possible to build the time series in
different ways where negative IPID differences are never observed, but in this
study our time series was the differences in the client's IPIDs in the order in
which they arrived at the measurement machine.  Our range of $[-40, 0)$ or $(0,
1000]$ is based on our observations of noise typical of the real Internet.  The
IPID going up by $0$ is a degenerate case and means the IPID is not global.

Servers were chosen from three groups: Tor directory authorities, Tor bridges,
and web servers.  The ten Tor directory authorities were obtained from the Tor
source code and the same ten IPs were tested for every day of data.  Three Tor
bridges were collected daily both through email and the web.  Every day seven
web servers were chosen randomly from the top 1000 websites on the Alexa Top
1,000,000 list~\cite{alexa}.  All web server IPs were checked to make sure that
they stood up for at least 24 hours before being selected for measurement.
Furthermore, we checked that the client and server were both up and behaving as
assumed between every experiment (\emph{i.e.}, every five minutes).
%We also
%probe the client's IPID using alternating source IPs to ensure that the IPID is
%global throughout the experiment (Some operating systems, such as Linux, have
%sequential incrementing IPIDs that are per-IP and not shared globally). 

A round of experiments was a 24-hour process in which measurements were carried
out on the two measurement machines.  Each 24-hour period had 22 hours of
experiments and 2 hours of down time for data synchronization.  For each
measurement period on each of the two machines performing direct measurements,
ten server machines and ten client machines from the above process were chosen
for geographic diversity: 5 from China, 2 from countries in Asia that were not
China, 1 from Europe, and 2 from North America.  IP addresses were never reused
except for the Tor directory authorities, so that every 24-hour period was
testing a set of 20 new clients, 10 new servers, and the 10 directory
authorities. 

For each of the twenty clients and twenty servers geographical information
provided by MaxMind was saved. MaxMind claims an accuracy of 99.8\% for identifying
the country an IP address is in~\cite{maxmindaccuracy}.  For each of the twenty
server machines, a series of SYN packets was used to test and save its SYN/ACK
retransmission behavior for the analysis in Section~\ref{sec:analysis}.

Every hour, each of our two main measurement machines created ten threads.
Each thread corresponded to one client machine.  Each thread tested each of the
ten server IP addresses sequentially using our idle scan based on the client's
IPID.  No forged SYNs were sent to the server during the first 100 seconds of a
test, and forged SYNs with the return IP address of the client were sent to the
server at a rate of 5 per second for the second 100-second period.  Then forged
RST packets were sent to the server to clear the SYN backlog and prevent
interference between sequential experiments.  A timeout period of sixty seconds
was observed before the next test in the sequence was started, to allow all
other state to be cleared.  Each experiment lasted for less than five minutes,
so that ten could be completed in an hour.  Every client and server was
involved in only one experiment at a time.  Each client/server pair was tested
once per hour throughout the 24-hour period, for replication and also to
minimize the effects of diurnal patterns.  Source and destination ports for all
packets were carefully chosen and matched to minimize assumptions about what
destination ports the client responds on.  Specifically, source ports for SYN
packets sent to the server (both forged SYNs and SYNs with the measurement
machine's IP address as the return IP address for testing) were chosen from the
same range as the destination ports for SYN/ACKs send to the client (always
strictly less than 1024).  We did not find it necessary to hold the source port
for SYN/ACKs sent to the client to be always equal to the open port on the
server, but this is possible.

In this section, we set out our statistical model for our time series data.
We then describe our process for outlier removal and for statistically
testing if and in which direction packet drops are occurring.

We model each time series $y_1, \ldots, y_n$ as a \emph{linear regression with
ARMA errors}, a combination of an autoregressive-moving-average (ARMA) model
with external linear regressors.  ARMA models are used to analyze time series
with autocorrelated data and are themselves a combination of two models, an
autoregressive (AR) model and a moving-average (MA) model.

An AR model of order $p$ specifies that every element of a time series can be
written as a constant plus the linear combination of the previous $p$ elements:
\[
y_t = c + z_t + \phi_1 y_{t-1} + \cdots + \phi_{t-p} y_{t-p}
\]
where $z_t$ is a white noise series.  An MA model of order $q$ specifies that
every element of a time series can be written as a constant plus the linear
combination of the previous $q$ white-noise terms:
\[
y_t = c + z_t + \theta_1 z_{t-1} + \cdots + \theta_{t-q} z_{t-q}
\]
Intuitively, each element is linearly related to the previous random ``shocks''
in the series.  An ARMA($p$, $q$) model combines an AR model of order $p$ and
an MA model of order $q$:
\[
y_t = c + z_t + \sum_{i=1}^p\phi_i y_{t-i} + \sum_{i=1}^q\theta_i z_{t-i}
\]

We use a linear regression with ARMA errors to model our time series data.
This specifies that every element in a time series can be written as a constant
plus the linear combination of regressors $x_1, \ldots, x_r$ with an
ARMA-modeled error term:
\begin{align*}
y_t &= c + \sum_{i=1}^r\beta_i x_{it} + e_t,\\
e_t &= z_t + \sum_{i=1}^p\phi_i e_{t-i} + \sum_{i=1}^q\theta_i z_{t-i}
\end{align*}

We use the regressors $x_i$ for \emph{intervention analysis}, \emph{i.e.}, for
analyzing our experimental effect on the time series at a specific time.

\begin{diagramsure*}[t!]
  \centering
  \includegraphics[width=0.95\textwidth]{diagrams/model-crop.pdf}
  \caption{{\bf For a server that retransmits $r-1$ SYN/ACK's, each case can be
expressed as the linear combination of regressors $x_1, \ldots, x_r$; shown is
when $r=3$ with SYN/ACK transmissions responding to the first forged SYN
occurring at $t_1$, $t_2$, and $t_3$.  C$\rightarrow$S indicates
client-to-server, and S$\rightarrow$C indicates
server-to-client.}\label{diagrams:model}} \end{diagramsure*}

For each experiment, we pick regressors according to which times the server
(re)transmits SYN/ACK's in response to SYN's.  For a server that (re)transmits
$r$ SYN/ACK's in response to each SYN, we have $r$ regressors.  We call time
$t_1$ the time of the first transmission in response to the first of our forged
SYN's, and we call $t_{i+1}$ the time the server would send the $i$th
retransmission in response to that SYN.  Then we define regressor $x_i$ as the
indicator variable
\begin{align*}
x_{ij} =
\begin{cases}
1 &\textnormal{if $t_i \le j$ and either $j < t_{i+1}$ or $i = r$}\\
0 &\textnormal{otherwise}
\end{cases}
\end{align*}
In other words, $x_1$ is zeros until the time the server transmits the first
SYN/ACK then ones until the server begins retransmitting SYN/ACK's.  The
remaining $x_i$ are zeros until the time the server would begin retransmitting
its $i$th SYN/ACK then ones until if/when the $(i+1)$th SYN/ACK's would begin
being retransmitted.  This definition allows us to model any of the possible
level shifts in any case of packet drop as a linear combination of all $x_i$.
See diagramsure~\ref{fig:model} for an illustration.

We choose ARMA orders $p$ and $q$ by performing model selection over time
series elements $y_1, \ldots, y_{t_1}$.  We find the $p\le7$ and $q\le7$
for the ARMA($p$, $q$) model that maximizes the corrected Akaike information
criterion, a metric which rewards models that lose less information but
penalizes models overfitted with too many parameters~\cite{aicc}.  It is given
by
\[
AIC_C = -2\ln{L} + 2k + \frac{2k(k+1)}{n-k-1},
\]
where here the number of parameters $k$ is $p + q + 2$ and where $L$ is the
estimated maximum likelihood over all $\phi_i$ and $\theta_i$.

After $p$ and $q$ are chosen, we then simultaneously fit all $\phi_i$,
$\theta_i$, and $\beta_i$ of our linear regression model with ARMA errors over
the entire time series $y_1, \ldots, y_n$ corresponding to the estimated
maximum likelihood.

After fitting parameters, we remove outliers that might be caused by,
\emph{e.g.}, spikes in network traffic that may hamper our analysis.  We use
the $\hat{\lambda}_{2,T}$ test statistic proposed by Chang \emph{et.\
al}~\cite{outliers} with significance $\alpha = 0.05$.  After removing
outliers, we iteratively refit the $\phi_i$, $\theta_i$, and $\beta_i$
parameters and test for outliers until no additional outliers are removed.

For intervention analysis, we use hypothesis testing over the value of
$\beta_r$ to determine if packets are dropped and in which direction.  If we
send $s$ forged SYN's, without noise, we would expect $\beta_r$ to equal one of
the following: $0$ for the case where packets are dropped from the server to
client, $s$ for the case where no packets are dropped, or $rs$ for the case
where packets are dropped from the client to server.  One might pick two
thresholds, $k_1 = s/2$ in between the first two cases and threshold $k_2 = (1
+ r)s/2$ between the last two cases; however, for the second threshold, we
instead choose $k_2' = \min(2s, k_2)$ to be more robust to, \emph{e.g.}, packet
loss.  Then we determine the case by a series of one-sided hypothesis tests
performed with significance $\alpha = 0.01$ according to the following
breakdown:

\begin{packed_item}
\item
\textbf{Server-to-client-dropped} if we reject the null hypothesis that
$\beta_r \ge k_1$.
\item
\textbf{No-packets-dropped} if we reject the null hypotheses that $\beta_r \le
k_1$ and that $\beta_r \ge k_2'$.
\item
\textbf{Client-to-server-dropped} if we reject the null hypothesis that
$\beta_r \le k_2'$.
\item \textbf{Error} if none of the above cases can be determined.
\end{packed_item}


Table~\ref{tab:results} shows results from 5 days of data collection, where $S
\rightarrow C$ is {\bf Server-to-client-dropped}, {\it None} is {\bf
No-packets-dropped}, $C \rightarrow S$ is {\bf Client-to-server-dropped}, and
{\it Error} is {\bf Error}.  {\it CN} is China, {\it Asia-CN} is other Asian
countries, {\it EU} is Europe, and {\it NA} is North America.  For server
types, {\it Tor-dir} is a Tor directory authority, {\it Tor-bri} is a Tor
bridge, and {\it Web} is a web server.

\begin{table}
\centering
\begin{footnotesize}
\begin{tabular}{ | c | c | c | c | c |}
\hline
\hline
\multicolumn{1}{c}{Client,Server} & 
\multicolumn{1}{c}{$S \rightarrow C$ (\%)} & 
\multicolumn{1}{c}{None (\%)} & 
\multicolumn{1}{c}{$C \rightarrow S$ (\%)} & 
\multicolumn{1}{c}{Error (\%)} \\
\hline
\hline
CN,Tor-dir & 2200 (73.04)  & 19 (0.63) & 504 (16.73) & 289 (9.59) \\
Asia-CN,Tor-dir & 0 (0.00)  & 1171 (96.38) & 1 (0.08) & 43 (3.54) \\
NA,Tor-dir & 1 (0.07)  & 1217 (90.69) & 49 (3.65) & 75 (5.59) \\
EU,Tor-dir & 2 (0.28)  & 695 (97.89) & 2 (0.28) & 11 (1.55) \\
CN,Tor-bri & 1012 (58.91)  & 565 (32.89) & 31 (1.80) & 110 (6.40) \\
Asia-CN,Tor-bri & 0 (0.00)  & 626 (80.88) & 9 (1.16) & 139 (17.96) \\
NA,Tor-bri & 0 (0.00)  & 657 (78.21) & 30 (3.57) & 153 (18.21) \\
EU,Tor-bri & 0 (0.00)  & 313 (78.25) & 9 (2.25) & 78 (19.50) \\
CN,Web & 28 (2.15)  & 995 (76.30) & 36 (2.76) & 245 (18.79) \\
Asia-CN,Web & 1 (0.17)  & 569 (97.43) & 1 (0.17) & 13 (2.23) \\
NA,Web & 0 (0.00)  & 606 (93.37) & 0 (0.00) & 43 (6.63) \\
EU,Web & 0 (0.00)  & 305 (90.24) & 0 (0.00) & 33 (9.76) \\
\hline
All Web & 29 (1.01)  & 2475 (86.09) & 37 (1.29)  & 334 (11.62) \\
All Tor-bri & 1012 (27.12)  & 2161 (57.90) & 79 (2.12)  & 480 (12.86) \\
All Tor-dir & 2203 (35.09)  & 3102 (49.40) & 556 (8.85)  & 418 (6.66) \\
\hline
\end{tabular}
\caption{Results from the measurement study.\label{tab:results}}
\end{footnotesize}
\end{table}

Our expectation would be to observe {\bf Server-to-client-dropped} for
clients in China and Tor servers because of Winter and Lindskog's observation
that the SYN/ACKs are statelessly dropped by the ``Great Firewall of China''
(GFW) based on source IP address and port~\cite{winter2012}.  We would expect
to see {\bf No-packets-dropped} for most web servers from clients in China,
unless they host popular websites that happen to be censored in China.
Similarly, in the expected case we should observe {\bf No-packets-dropped} for
clients outside of China, regardless of server type.  We expect a few
exceptions, because censorship happens outside of China and because
the GFW is not always 100\% effective.  In particular, Tor bridges are not
blocked until the GFW operators learn about them, and some routes might not
have filtering in place.  Our results are congruent with all of these
expectations. 

In 5.9\% of the client/server pairs we tested, multiple cases were observed in
the same day.  In some cases it appears that noise caused the wrong case to be
detected, but other cases may be attributable to routes changing throughout the
day~\cite{tcp5}.  That the data is largely congruent with our expectations
demonstrates the efficacy of the approach, and some of the data points that lie
outside our expectations have patterns that suggest that a real effect is being
measured, rather than an error.  For example, of the 28 data points where web
servers were blocked from the server to the client in China, 20 of those data
points are the same client/server pair. 
%Both the client and the server had no
%such issues in measurements with the other 9 servers/clients throughout the
%same 24-hour period, suggesting that for that client that particular server is
%indeed blocked.  Of the 20 cases where packets are dropped from client to
%server in China for web servers, 15 are the same client/server pair.

38\% of the data we collected does not appear in Table~\ref{tab:results}
because it did not pass liveness tests.  Every 5-minute data point has three
associated liveness tests.  If a server sends fewer than 2.5 SYN/ACKs in
response to SYNs from the measurement machine, a client responds to less than
$\frac{3}{5}$ of our SYN/ACKs, or a measurement machine sending thread becomes
unresponsive, that 5-minute data point is discarded.

Two out of the ten Tor directory authorities never retransmitted enough
SYN/ACKs to be included in our data.  Of the remaining eight, two more account
for 98.8\% of the data points showing blocking from client to server.
These same two directory authorities also account for 72.7\% of the {\bf Error}
cases for directory authorities tested from clients in China, and the case of
packets being dropped from server to client (the expected case for China and
the case of the majority of our results) was never observed for these two
directory authorities.

When Winter and Lindskog~\cite{winter2012} measured Tor reachability from a
virtual private server in China, there were eight directory authorities at that
time.  One of the eight was completely accessible, and the other seven were
completely blocked in the IP layer by destination IP (\emph{i.e.}, {\bf
Client-to-server}).  In our results, six out of ten are at least blocked {\bf
Server-to-client} and two out of ten are only blocked {\bf Client-to-server}
(two had all results discarded).  Winter and Lindskog also observed that Tor
relays were accessible 1.6\% of the time, and we observed that directory
authorities were accessible 0.63\% of the time.  Our results have geographic
diversity and their results can serve as a ground truth because they tested
from within China.  In both studies the same special treatment of directory
authorities compared to relays or bridges was observed, as well as a small
percentage of cases where filtering that should have occurred did not.

To evaluate the assumption that clients with a global IPID are easy to find in
a range of IP addresses that we desire to measure from, take China as an
example.  On average, 10\% of the IP addresses in China responded to our probes
so that we could observe their IPID, and of those 13\% were global.  So,
roughly 1\% of the IP address space of China can be used as clients for
measurements with our method, enabling experiments with excellent geographic
and topological diversity.




==> intro.tex <==
China and brief history of GFC. Explain why it is hard to know what they are doing. Why it is matter to know what is going on. 
Current works for china is mainly assume topology is an important factor, but no one investigate the geography of the IPs and possiblity that affect censorships as well. Why do we care about this. Expalin why not there is no research about the location (limitation on the widespread nodes).

Great Firewall of China is the biggest international firewall that exists. But it is not working always. This is observed through these research. Now the question is what are the main factors that affect the efficiency of chineese firewall(diunearl pattern, other themporal patterns, geographical route coverage issues). 

Our contribution is :
investigate that lack of topological centralization of censorships is a reason for inconsistancy,
ivestigate that how geography of IP matters


==> results.tex <==
Can we show at-least for linux based machine that in general, when a RST is blocked going from a
client in China to a Tor relay outside China then a SYN packet will also
be blocked, and when a RST is not blocked a SYN packer also will not be.
